MultiLegalSBD: A Multilingual Legal Sentence Boundary Detection Dataset

Sentence Boundary Detection (SBD) is one of the foundational building blocks of Natural Language Processing (NLP), with incorrectly split sentences heavily influencing the output quality of downstream tasks. It is a challenging task for algorithms, especially in the legal domain, considering the complex and different sentence structures used. In this work, we curated a diverse multilingual legal dataset consisting of over 130'000 annotated sentences in 6 languages. Our experimental results indicate that the performance of existing SBD models is subpar on multilingual legal data. We trained and tested monolingual and multilingual models based on CRF, BiLSTM-CRF, and transformers, demonstrating state-of-the-art performance. We also show that our multilingual models outperform all baselines in the zero-shot setting on a Portuguese test set. To encourage further research and development by the community, we have made our dataset, models, and code publicly available.

==> Content/_1-LegalSBD.tex <==
\section{Legal Sentence Boundary Detection}
\label{ch:LegalSBD}
%Too detailed?

Legal text offers an increased challenge to SBD-Systems because of the way it is structured. Often it consists of sections and subsections, quite different to formal text such as news article. Furthermore, more complex structures including headers, footnotes, citations and lists are part of the text and do not follow a standard sentence structure. Therefore, a different taxonomy for sentence structures in legal text has to be applied.
Below we describe the most important sentence structures in legal text followed by an example, heavily inspired by \citet{Savelka}:

\begin{description}
    \item[Standard Sentence] Subject, object and verb  are in the correct order and the last token in the sequence is a sentence-terminating character.
    \begin{description}
        \item \textit{Il s'est établi comme ingénieur indépendant.}
    \end{description}
    \item[Linguistically Transformed Sentence] Similar to a standard sentence, but slight transformations such as a change of the word order are applied.
    \begin{description}
        \item\textit{Tout porte à croire, en réalité, qu'elle est condamnée au surendettement, puis à la faillite.}
    \end{description}
    \item[Headlines] Determine the structure of the text and show relatedness between parts of the document and therefore convey important information about the overall structure of the text.
    \begin{description}
        \item\textit{Considérant en fait et en droit}
        \item\textit{Article 9-1}
        \item\textit{PAR CES MOTIFS}
        \item\textit{DÉCLARATION}
    \end{description}
    \item[Citations] Links different documents as well as passages inside the text. This type of structure appears often in legal text.
    \begin{description}
        \item \textit{Au 2°, les mots: "ou de la cellule de recueil, de traitement et d'évaluation des informations préoccupantes relatives aux mineurs en danger ou qui risquent de l'être, mentionnée au deuxième alinéa de l'article L. 226-3 du code de l'action sociale et des familles," sont supprimés.}

    \end{description}
    \item[Lists] Annotated differently depending on the type of list. For lists with incomplete sentences as list items the whole list up to the first sentence terminating character is annotated as a sentence. The following example consists of 2 sentences, the introductionary sentence and the list itself:
    \begin{description}
        \item \textit{Au cours du délai fixé par la juridiction pour accomplir un travail d'intérêt général, le condamné doit, outre l'obligation d'accomplir le travail prescrit, satisfaire aux mesures de contrôle suivantes:\\
        1° Répondre aux convocations du juge de l'application des peines ou du travailleur social désigné;\\
        2° Se soumettre à l'examen médical préalable à l'exécution de la peine qui a pour but de rechercher s'il n'est
        pas atteint d'une affection dangereuse pour les autres travailleurs et de s'assurer qu'il est médicalement apte
        au travail auquel il est envisagé de l'affecter.}
    \end{description}
    However, if the list items themselves are sentences, the list number or letter and the list items are both annotated as one sentence each. In the example below, we have 2 sentences with "A.-" and the list item being annotated separately.
    \begin{description}
        \item \textit{A.- D.\_ est entré à l'école de recrues le 16 juillet 1979.}
    \end{description}
    \item[Ellipses] Used to indicate when part of a sentence or a full sentence are left out. 
    The following example shows the use cases for ellipses. The first ellipsis is annotated separately, as it indicates a sentence or sentences that are missing. The second ellipses indicates, that part of that single sentence was left out and is therefore not annotated separately.
    \begin{description}
        \item \textit{(...) La faute de X. est d'une exceptionnelle gravité tant les faits qui lui sont reprochés (...), commis avec une certaine froideur sont insoutenables et comportent un caractère insupportable pour les victimes.}
    \end{description}
    \item[Parentheses] Similar to citations and they often appear together. They are used to link to passages of different documents. The parentheses inside a sentence are annotated as part of the sentence. Even if a complete, different sentence should appear inside the parentheses, it is annotated as part of the overall sentence.
    \begin{description}
        \item \textit{Le recourant ne saurait se contenter de soulever de vagues griefs ou de renvoyer aux actes cantonaux (ATF 122 I 70 consid. 1c; 121 IV 317 consid. 3b; 119 Ia 197 consid. 1d).}
    \end{description}
\end{description}

%Move tokenizer to section 4 or even section 5?





